Riemannian Functional Map Synchronization for Probabilistic Partial Correspondence in Shape Networks

We consider the problem of graph-matching on a network of 3D shapes with uncertainty quantification. We assume that the pairwise shape correspondences are efficiently represented as \emph{functional maps}, that match real-valued functions defined over pairs of shapes. By modeling functional maps between nearly isometric shapes as elements of the Lie group $SO(n)$, we employ \emph{synchronization} to enforce cycle consistency of the collection of functional maps over the graph, hereby enhancing the accuracy of the individual maps. We further introduce a tempered Bayesian probabilistic inference framework on $SO(n)$. Our framework enables: (i) synchronization of functional maps as maximum-a-posteriori estimation on the Riemannian manifold of functional maps, (ii) sampling the solution space in our energy based model so as to quantify uncertainty in the synchronization problem. We dub the latter \emph{Riemannian Langevin Functional Map (RLFM) Sampler}. Our experiments demonstrate that constraining the synchronization on the Riemannian manifold $SO(n)$ improves the estimation of the functional maps, while our RLFM sampler provides for the first time an uncertainty quantification of the results.

==> Sections/EuclidCalc.tex <==
\section{Computation on Euclidean Space}
\Faria{May need to delete this part?}

To benchmark our method, we will look into the corresponding results in euclidean space. For example, to compute MCMC on euclidean space, we can rewrite \cref{eq:MCMC} as follows:

\begin{align}
\mathbf{V}_i^{(k+1)} &=  h \nabla_{\Cm_i} U(\Cm_i^{(k)}) + \sqrt{2 h/\beta} \mathbf{Z}_i^{(k+1)} \\ 
\Cm_i^{(k+1)}  &= \Cm_i^{(k)} + \mathbf{V}_i^{(k+1)}, \hspace{30pt} \forall i \in \{1,\dots,n\},  
\end{align}

As in this case, we are not constrained to reside on top of the SO group anymore, we can get rid of the \textit{projection} $\Pi$ and \textit{retraction} $R$ here. The update function hence becomes simpler than before. 

==> Sections/GradientCalc.tex <==
\section{Computation of the gradient of U}

\paragraph{Preliminary} Consider the function: \tolga{why is this $(p,p)$? is the functional map always square? then it is just an orthogonal matrix? And usually, I use the bold for matrix notation and calligraphic to denote the set. But this is conventional.} $f: St(p, p) \rightarrow \mathbb{R}$ defined by:
$$f(X) = d^2(X, C_1)$$
where $d^2$ is the squared geodesic distance associated with the canonical Riemannian metric on the SO group $St(p, p)$.

The gradient of $f$ at $X \in St(p, p)$ is an element of $T_X(St(p, p))$ and defined as:
$$\nabla_Xf = - 2 . \text{Log}_X(C_1),$$
where Log is the Riemannian logarithm associated with the canonical Riemannian metric on the SO group $St(p, p)$.\\

\paragraph{Gradient of $U$} We will use this result to compute the gradient of $U: St(p, p)^{n-1} \rightarrow \mathbb{R}$ defined on $n-1$ copies of the SO group $St(p, p) \times ... \times St(p, p)=St(p, p)^{n-1}$ as:
%\begin{strip}
\begin{align*}
U(\mathbf{C}) 
    &= U(C_2, ..., C_n) \\
    &= \sum_{i, j \in \mathcal{E}} 
        d^2(C_i^{-1}.C_j, C_{ij})\\
    &= \sum_{i, j \in \mathcal{E}} 
        d^2(C_j, C_i.C_{ij}) 
        %\quad \text{ using the fact that: } \forall B, X_1, X_2 \in St(p, p), d(B.X_1, B.X_2) = d(X_1, X_2) \text{ with $B=C_i$.}
\end{align*}
%\end{strip}

using the fact that: $\forall B, X_1, X_2 \in St(p, p), d(B.X_1, B.X_2) = d(X_1, X_2)$ with $B=C_i$.

We consider $U$ as a function of $\mathbf{C} \in St(p, p)^{n-1}$, where $\mathbf{C}$ has shape $p \times (n-1)p$, that is taking values in $\mathbb{R}$. The gradient of $U$ at $\mathbf{C}^0= (C_2^0, ..., C_n^0)$, written $\nabla_{\mathbf{C}^0}U$ can be represented as matrix of shape $p \times (n-1)p$ as:
$$\nabla_{\mathbf{C}^0}U 
= \frac{\partial U}{\partial \mathbf{C}}(\mathbf{C}^0)
= \left(
\frac{\partial U}{\partial C_2}(\mathbf{C}^0), ...\frac{\partial U}{\partial C_n}(\mathbf{C}^0)\right),
$$
which is used to compute the directional derivative at $\mathbf{C}^0$ in the direction $S \in T_{\mathbf{C}^0}St(p, p)^{n-1}$, where $S$ a matrix of size $p \times (n-1)p$ in the tangent space of $St(p, p)^{n-1}$ at $\mathbf{C}^0$ as:
\begin{equation}
    DU_{\mathbf{C}^0}(S) = \nabla_{\mathbf{C}^0}U \cdot S = \text{Tr}\left((\nabla_{\mathbf{C}^0}U)^T.S\right)
\end{equation}
where we use the notation $\cdot$ to represent the Frobenius inner product of matrices.\\

Thus, we need to compute each $\frac{\partial U}{\partial C_k}(\mathbf{C}_0)$, for $k \in \{2, ..., n\}.$\\

We have \dena{should break properly to fit in double column}:
\begin{strip}

\begin{align*}
\frac{\partial U}{\partial C_k}(\mathbf{C}_0)
&= \frac{\partial}{\partial C_k} \left(
    \sum_{i, j \in \mathcal{E}} d^2(C_i^{-1}.C_j, C_{ij})\right)(
        \mathbf{C}_0)\\
&= \frac{\partial}{\partial C_k}\left(
    \sum_{j \text{ linked to } k }d^2(C_k^{-1}.C_j, C_{kj}) + 
    \sum_{i \text{ linked to } k } d^2(C_i^{-1}.C_k, C_{ki})\right)(
        \mathbf{C}_0)\\
&= 
    \sum_{j \text{ linked to } k } \frac{\partial}{\partial C_k} d^2(C_k^{-1}.C_j, C_{kj})(
        \mathbf{C}_0)
    + \sum_{i \text{ linked to } k }  \frac{\partial}{\partial C_k}d^2(C_i^{-1}.C_k, C_{ki})(
        \mathbf{C}_0)\\    
\end{align*}

\end{strip}
Note that the expression in parenthesis (as a function of $C_2, ..., C_n$ without $C_k$) is a composition of linear operations (matrix multiplication), a geodesic squared distance ($d^2$) and a sum of such functions: these operations preserve the convexity of the functions, thus the result is a convex function. (to prove mathematically?).\\


Thus, we need to define the gradients of the functions $g_j: St(p, p)\rightarrow \mathbb{R}$ defined as:
%$$g_j(C_k) = d^2(C_k^{-1}.C_j, C_{kj}) = d^2(C_j, C_k.C_{kj}) = d^2(C_k.C_{kj}, C_j)  \quad \text{ bcs } d^2(C.X_1, C.X_2) = d^2(X_1, X_2) ,$$

\begin{align*}
g_j(C_k) 
&= d^2(C_k^{-1}.C_j, C_{kj}) \\
&= d^2(C_j, C_k.C_{kj}) \\
&= d^2(C_k.C_{kj}, C_j) \text{ $bcs$ } d^2(C.X_1, C.X_2) \\
&= d^2(X_1, X_2),
\end{align*}

and of the functions $h_i: St(p, p)\rightarrow \mathbb{R}$ defined as:
$$h_i(C_k) = d^2(C_i^{-1}.C_k, C_{ki}).$$

\paragraph{Gradient of $h_i$} 

To compute the gradient of $h_i$ we use the chain rule by considering: $h_i = f \circ \Tilde{h_i}$ where:
\begin{align*}
    \tilde{h_i}: St(p, p) &\rightarrow St(p, p)\\
    X &\rightarrow C_i^{-1}.X
\end{align*}
and:
\begin{align*}
    f: St(p, p) &\rightarrow \mathbb{R}\\
    Y &\rightarrow d^2(Y, C_{ki})
\end{align*}

We have the gradient of the $\tilde{h_i}$ that writes: $\nabla_{C_0}\tilde{h_i} = C_i^{-1}$. Additionally, the gradient of $f$ is given by the preliminary. The chain rule, written in terms of the directional derivative at $C_k^0$ in the direction $S \in T_{C_k^0}St(p, p)$ gives:
\begin{align*}
    D_{C_k^0}(f \circ \Tilde{h_i})(S)
    &= D_{\Tilde{h_i}(C_k^0)}f\circ D_{C_k^0}(S)\\
    &= D_{(C_i^{-1}C_k^0)}f(C_i^{-1}.S)\\
    &= D_{C_i^{-1}C_k^0}f(C_i^{-1}.S)\\
    &= - 2 . \text{Log}_{C_i^{-1}C_k^0}(C_{ki}) \cdot C_i^{-1}S \\ %\quad \text{using $\cdot$ as the Frobenius inner product}\\
    &= - 2 . \text{Tr}\left((\text{Log}_{C_i^{-1}C_k^0}(C_{ki}))^T.(C_i^{-1}S)\right)\\
    &= - 2 . \text{Tr}\left((\text{Log}_{C_i^{-1}C_k^0}(C_{ki}))^T.(C_i^TS)\right)\\
    &= - 2 . \text{Tr}\left((C_i.\text{Log}_{C_i^{-1}C_k^0}(C_{ki}))^T.S\right)\\
    &= - 2 . C_i. \text{Log}_{C_i^{-1}C_k^0}(C_{ki}) \cdot S
\end{align*}

using $\cdot$ as the Frobenius inner product.

Therefore, we can read in the above expression the gradient of $h_i$ at $\mathbf{C}_0$ is defined as:
$$\nabla_{\mathbf{C}_0}h_i 
= - 2 . C_{i0} . \text{Log}_{C_{i0}^{-1}C_{k0}}C_{ki}$$


